SparseFed: Mitigating Model Poisoning Attacks in Federated Learning with Sparsification

Federated learning is inherently vulnerable to model poisoning attacks because its decentralized nature allows attackers to participate with compromised devices. In model poisoning attacks, the attacker reduces the model's performance on targeted sub-tasks (e.g. classifying planes as birds) by uploading "poisoned" updates. In this report we introduce \algoname{}, a novel defense that uses global top-k update sparsification and device-level gradient clipping to mitigate model poisoning attacks. We propose a theoretical framework for analyzing the robustness of defenses against poisoning attacks, and provide robustness and convergence analysis of our algorithm. To validate its empirical efficacy we conduct an open-source evaluation at scale across multiple benchmark datasets for computer vision and federated learning.

==> macros.tex <==
\newcommand{\OblFt}{\mathbf{OblFtrSel}}
\newcommand{\FullFt}{\mathbf{FullFtrSel}}

\newcommand{\OblRisk}{\mathbf{OblRisk}}
\newcommand{\FullRisk}{\mathbf{FullRisk}}

\newcommand{\LearnFtr}{\mathsf{FtrSelector}}
\newcommand{\inj}{\mathsf{inj}}
\newcommand{\elim}{\mathsf{elim}}
\newcommand{\sub}{\mathsf{sub}}

\newcommand{\add}{\mathsf{add}}
\newcommand{\rem}{\mathsf{rem}}
\newcommand{\flip}{\mathsf{flip}}


\newcommand{\pop}{\mathsf{pop}}
\newcommand{\targ}{\mathsf{targ}}

\newcommand{\Advan}{\mathrm{Adv}}




\newcommand{\sanjam}[1]{}%{{[{\color{red} \bf Sanjam: #1}]}}
\newcommand{\sedits}[1]{}%{{{\color{magenta} #1}}}
\newcommand{\FT}[1]{}%{{[{\color{blue} \bf Florian: #1}]}}
\newcommand{\SJ}[1]{}%{{[{\color{purple} \bf Somesh: #1}]}}

\newcommand{\Mnote}[1]{}%{{\color{red}[{\bf Mohammad:}  #1]}}
\newcommand{\MohNote}[1]{}%{{\color{red} [{\bf Mohammad:}  #1]}}

%\newcommand{\SomNote}[1]{}{{\color{purple} [{\bf Somesh:}  #1]}}

\newcommand{\SaeedNote}[1]{}%{{[{\color{teal} \bf Saeed: #1}]}}
\newcommand{\Snote}[1]{}%{\SaeedNote{#1}}

\newcommand{\AbhrNote}[1]{}%{{\color{red} [{\bf Abhradeep:}  #1]}}
\newcommand{\SamNote}[1]{}%{{\color{orange} [{\bf Sam:}  #1]}}
\newcommand{\SNote}[1]{}%{{\color{green} [{\bf Shuang:}  #1]}}


% \newcommand{\nicholas}[1]{{[{\color{green} \bf Nicholas: #1}]}}



% \usepackage{enumitem}

% \usepackage{centernot}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\fot}{\bff}
\newcommand{\fto}{\bfg}
\newcommand{\htet}{\hat{\theta}}

\newcommand{\fhat}[2]{\ifthenelse{\equal{#2}{}}{\hat{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\hat{f}(\emptyset)}{\hat{f}(#1_{\leq #2})}}}
\newcommand{\ftild}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f}(\emptyset)}{\tilde{f}(#1_{\leq #2})}}}
\newcommand{\ftildstar}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f^*}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f^*}(\emptyset)}{\tilde{f^*}(#1_{\leq #2})}}}
\newcommand{\ghat}[2]{\ifthenelse{\equal{#2}{}}{\hat{g}(#1)}{\ifthenelse{\equal{#2}{0}}{\hat{g}(\emptyset)}{\hat{g}(#1_{\leq #2})}}}
\newcommand{\mfix}[2]{\ifthenelse{\equal{#2}{}}{m(#1)}{\ifthenelse{\equal{#2}{0}}{m(\emptyset)}{m(#1_{\leq #2})}}}


\newcommand{\fapp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f}(\emptyset)}{\tilde{f}(#1_{\leq #2})}}}

\newcommand\aug{\hspace{-2.5mm}\rule[-1mm]{0.1mm}{4.5mm}\hspace{-2.5mm}}
\newcommand\augp{\hspace{-2.5mm}\rule[-2mm]{0.1mm}{5mm}\hspace{-2.5mm}}
\newcommand\augt{\hspace{-2.5mm}\rule[-1mm]{0.1mm}{5mm}\hspace{-2.5mm}}
\newcommand{\concatt}[4]{\begin{bmatrix}
\vspace{-5mm}\\
   #1&\augp&#2\\
   #3&\augt&#4\\
   \vspace{-5mm}\\
    \end{bmatrix}}
\newcommand{\concat}[2]{\begin{bmatrix}
\vspace{-5mm}\\
   #1&
   \aug
   &#2\\
   \vspace{-5mm}\\
    \end{bmatrix}}
\newcommand{\concatv}[2]{\begin{bmatrix}
   #1\\
   #2\\
    \end{bmatrix}}
    
    \newcommand{\concatvv}[3]{\begin{bmatrix}
   #1\\
   #2\\
   #3\\
    \end{bmatrix}}

%\newcommand{\gain}[2]{\ifthenelse{\equal{#2}{}}{g[#1]}{g[#1_{\leq #2}]}}


% CONVENTION for VECTOR and DISTRIBUTION notation:  
%For x,y,z, use \xDist \yDist etc to get their distribution, for d exceptionally use just \dist. for their vector version add Vec at the end of these operations or just get \xVec to get the vector that is not a distribution
%\newcommand{\againAp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{g}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{g}(\emptyset)}{\tilde{g}({#1}_{\leq #2})}}}
\renewcommand{\t}{\mathsf{t}}
% \renewcommand{\Case}{\mathrm{C}}
\newcommand{\Otilde}{\wt{O}}
\newcommand{\PrTam}{\mathsf{PT}}

\newcommand{\metric}{{{\mathsf{d}}}}
\newcommand{\metr}{\metric}
\newcommand{\Ball}{\mathcal{B}all}
\newcommand{\Sph}{\mathcal{S}phr}

\newcommand{\diam}{\mathsf{Diam}}
% \usepackage[utf8]{inputenc}
\newcommand{\Levy}{Lévy\xspace}
\newcommand{\Lovasz}{Lovász\xspace}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\paragcompact}[1]{\noindent{\bf #1}}

%\newcommand{\parag}[1]{\noindent{\bf #1}}
%\renewcommand{\paragraph}[1]{\parag{#1}}
\newcommand{\distdist}{\mathfrak{D}}

%\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace} % X
%\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace} % X

\newcommand{\HD}{\mathsf{HD}}
\newcommand{\con}{{\bm \upalpha}}
\newcommand{\ERM}{\mathsf{ERM}}

\newcommand{\msr}{{\bm{\upmu}}}
\newcommand{\CentDist}{{\bm{\upsigma}}}

\newcommand{\OnlTam}{\mathsf{On}\Tam}
\newcommand{\OnTam}{\OnlTam}
\newcommand{\OffTam}{\mathsf{Off}\Tam}
%\newcommand{\OnlTam}{\OnlTam}
%\newcommand{\OnTam}{\OnTam}
%\newcommand{\OffTam}{\OffTam}

\newcommand{\mal}{\wt}
\newcommand{\X}{\cX} % X
\newcommand{\Y}{\cY} % X
%\newcommand{\msr}{{\mathbf{D}}}
%\newcommand{\dist}{\mathbf{d}}
%\newcommand{\dDist}{\dist}
%\newcommand{\dVec}{\ol{d}}
%\newcommand{\distVec}{\ol{\dist}}
\newcommand{\hypo}{h}
%\newcommand{\Dist}{\msr}
\newcommand{\C}{\cC}
\newcommand{\D}{\cD}
\renewcommand{\H}{\cH}
\newcommand{\error}{\mathsf{Err}}
\newcommand{\Error}{\error}
\newcommand{\Conf}{\mathsf{Conf}}
\newcommand{\conf}{\Conf}
\newcommand{\alphaDist}{{\bm \upalpha}}
\newcommand{\Risk}{\mathsf{Risk}}
\newcommand{\Rob}{\mathsf{Rob}}



\newcommand{\Tam}{\mathsf{Tam}}
\newcommand{\TamAb}{\mathsf{TamAb}}
\newcommand{\AppTam}{\mathsf{AppTam}}
\newcommand{\AppTamAb}{\mathsf{AppTamAb}}
%\newcommand{\ORTam}{\mathsf{ORSam}}
%\newcommand{\KRTam}{\mathsf{KRSam}}
\newcommand{\Inv}{\mathsf{Inv}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Trans}{\mathsf{Trans}}
\newcommand{\Small}{\mathsf{Small}}
\newcommand{\UnBal}{\mathsf{UnBal}}
\newcommand{\Good}{\mathsf{Good}}
\newcommand{\High}{\mathrm{High}}
\newcommand{\Low}{\mathrm{Low}}
\newcommand{\BigOut}{\mathrm{Big}}
\newcommand{\SmallOut}{\mathrm{Small}}


\newcommand{\xDist}{\mathbf{x}}
\newcommand{\yDist}{\mathbf{y}}
\newcommand{\zDist}{\mathbf{z}}
\newcommand{\tDist}{\mathbf{t}}
\newcommand{\TDist}{\mathbf{T}}
\newcommand{\WDist}{\mathbf{W}}
\newcommand{\sDist}{\mathbf{s}}
\newcommand{\uDist}{\mathbf{u}}
\newcommand{\vDist}{\mathbf{v}}
\newcommand{\wDist}{\mathbf{w}}



\newcommand{\XDist}{\mathbf{X}}
\newcommand{\UDist}{\mathbf{U}}
\newcommand{\trainDist}{\UDist}

\newcommand{\xDistVec}{\ol{\xDist}}
\newcommand{\yDistVec}{\ol{\yDist}}
\newcommand{\zDistVec}{\ol{\zDist}}
\newcommand{\tDistVec}{\ol{\tDist}}
\newcommand{\sDistVec}{\ol{\sDist}}
\newcommand{\uDistVec}{\ol{\uDist}}
\newcommand{\vDistVec}{\ol{\vDist}}
\newcommand{\wDistVec}{\ol{\wDist}}


\newcommand{\insDist}{\xDist}
\newcommand{\instDist}{\insDist}

\newcommand{\xVec}{\ol{x}}
\newcommand{\yVec}{\ol{y}}
\newcommand{\zVec}{\ol{z}}
\newcommand{\tVec}{\ol{t}}
\newcommand{\sVec}{\ol{s}}
\newcommand{\uVec}{\ol{u}}
\newcommand{\vVec}{\ol{v}}
\newcommand{\wVec}{\ol{w}}

\newcommand{\alVec}{{\ol{\alpha}}}
\newcommand{\alK}{{\bfK_\alVec}}
\newcommand{\alk}{{\bfK_\alVec}}
\newcommand{\alHD}{\HD_{\alVec}}

\newcommand{\SDist}{\mathbf{S}}

\newcommand{\uRP}{{\wt{\uDist}}}

\renewcommand{\th}{^\mathrm{th}}
\newcommand{\jointSamp}[2]{\langle #1 \,\, \| \, {#2}\rangle}
\newcommand{\fvers}{(Please see the full version for the proof.) }

\newcommand{\overbar}[1]{\mkern 1.9mu\overline{\mkern-2.9mu#1\mkern-0.5mu}\mkern 1.9mu}
\newcommand{\overbarr}[1]{\mkern 1.9mu\overline{\mkern-0.9mu#1\mkern-3.5mu}\mkern 1.9mu}
%\newcommand{\X}{\overbar{X}}
%\newcommand{\Y}{\overline{Y}}
%\newcommand{\Yd}{\overbarr{Y_\delta}}
%\newcommand{\Z}{\overbar{Z}}

%\renewcommand{\R}{\olverline{R}}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newcommand{\spn}{\mathrm{Span}}
\newcommand{\EQref}[1]{Equation~(\ref{#1})}
\newcommand{\VP}{\mathrm{ValPrf}}
\newcommand{\EX}{\mathsf{Ext}}
\newcommand{\Dn}{D^{\scriptscriptstyle (n)}}

\newcommand{\cost}{\mathsf{cost}}
\newcommand{\avgcost}{\overline{\cost}}


\newcommand{\KLsimp}{D_\mathsf{\scriptscriptstyle KL}}
\newcommand{\KL}[2]{D_\mathsf{\scriptscriptstyle KL}(#1||#2)}
\newcommand{\KLn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle KL}(#1||#2)}

\newcommand{\MDsimp}{D_{\scriptscriptstyle \infty}}
\newcommand{\MD}[2]{D_{\scriptscriptstyle \infty}(#1||#2)}
\newcommand{\MDn}[2]{D^{\scriptscriptstyle (n)}_{\scriptscriptstyle\infty}(#1||#2)}

\newcommand{\SDsimp}{D_\mathsf{\scriptscriptstyle SD}}
\newcommand{\SD}[2]{D_\mathsf{\scriptscriptstyle SD}(#1,#2)}
\newcommand{\SDn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle SD}(#1,#2)}

\newcommand{\minE}[1]{\mathrm{H}_{\scriptscriptstyle \infty}(#1)}

\newcommand{\pfix}[2]{ {#1}_{\leq #2}}
\newcommand{\pofix}[2]{#1_{\geq #2 }}
\newcommand{\dmax}{\mathsf{max}_\delta}
%\newcommand{\avr}[2]{\Ex[#1(#2)]}
\newcommand{\dMax}{\mathsf{Max}_{\geq \delta}}
\newcommand{\dlMax}{\mathsf{Max}_{< \delta}}

\newcommand{\Exists}{\exists\,}
\newcommand{\Forall}{\forall\,}
\newcommand{\fDist}{\mathbf{f}}
\newcommand{\aSF}{\mathsf{a}}
\newcommand{\gSF}{\mathsf{g}}
\newcommand{\hSF}{\mathsf{h}}

\newcommand{\avr}[2]{\ifthenelse{\equal{#2}{}}{\aSF({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF(\emptyset)}{\aSF({#1}_{\leq #2})}}}

\newcommand{\avrMax}[2]{\ifthenelse{\equal{#2}{}}{\aSF^*({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF^*(\emptyset)}{\aSF^*({#1}_{\leq #2})}}}

\newcommand{\avrApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}(\emptyset)}{\tilde{\aSF}({#1}_{\leq #2})}}}

\newcommand{\avrAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}^*({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}^*(\emptyset)}{\tilde{\aSF}^*({#1}_{\leq #2})}}}

\newcommand{\ArgMax}[2]{\ifthenelse{\equal{#2}{}}{\hSF({#1})}{\ifthenelse{\equal{#2}{0}}{\hSF(\emptyset)}{\hSF({#1}_{\leq #2})}}}

\newcommand{\AppArgMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\hSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\hSF}(\emptyset)}{\tilde{\hSF}({#1}_{\leq #2})}}}

\newcommand{\Err}{\mathcal{E}}
\newcommand{\expectedsub}[2]{\ensuremath{\mathop{{}\mathbf{E}}_{#1}\left[#2\right]}\xspace}
\newcommand{\charac}{\mathbf{1}}


\newcommand{\gain}[2]{\ifthenelse{\equal{#2}{}}{\gSF(#1)}{\gSF(#1_{\leq #2})}}
\newcommand{\gainMax}[2]{\ifthenelse{\equal{#2}{}}{\gSF^*(#1)}{\gSF^*(#1_{\leq #2})}}
\newcommand{\gainApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}(#1)}{\tilde{\gSF}(#1_{\leq #2})}}
\newcommand{\gainAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}^*(#1)}{\tilde{\gSF}^*(#1_{\leq #2})}}

%\newcommand{\avGain}(3]{{\mathcal{G}}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avAbGain}(3]{\mathcal{A}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avSqGain}(3]{\mathcal{Q}_{#3}(#1_{\leq #2 -1}]}



\newcommand{\RTam}{\mathsf{RejSam}}
\newcommand{\RTamk}{\mathsf{RejSam}_{k}}
%\newcommand{\RTamd}{\mathsf{RSam}_\delta}


\newcommand{\var}[2]{\Var[#1(#2)]}

\newcommand{\pr}[2][]{\Pr_{\ifthenelse{\isempty{#1}}{}{{#1}}}\left[{#2}\right]}

\newcommand{\GTam}{\mathsf{GTam}}
\newcommand{\EGTam}{\mathsf{EGTam}}

\newcommand{\LimSup}{\operatorname{limSup}}
%\newcommand{\sup}{\operatorname{sup}}
\newcommand{\pmbits}{\{+1,-1\}}
\newcommand{\pmint}{[-1,+1]}
%\newcommand{\Tam}{\Tam}
\newcommand{\IdealTam}{\mathsf{IdTam}}
\newcommand{\EffTam}{\mathsf{EffTam}}




% Oracle subroutines
\newcommand{\distO}{\mathbf{O}}
\newcommand{\setup}{\mathsf{G}}
\newcommand{\findsk}{{\mathsf{G}^{-1}}}
\newcommand{\enc}{\operatorname{Enc}}
\newcommand{\dec}{\operatorname{Dec}}
\newcommand{\rev}{\mathsf{rev}}
\newcommand{\decFull}{\operatorname{DecFull}}
\newcommand{\eval}{\mathsf{eval}}
\newcommand{\gi}{\mathsf{gi}}
\newcommand{\gc}{\mathsf{gc}}

\newcommand{\kgen}{\mathsf{K}}
\newcommand{\test}{\mathsf{T}}
\newcommand{\testatt}{mathsf{T}}
\newcommand{\V}{\mathsf{V}}
\newcommand{\Pred}{\mathsf{P}}
\newcommand{\Func}{\mathsf{F}}

% Garbling and RE
\newcommand{\lbl}{\mathsf{label}}
\newcommand{\GCircuit}{\mathsf{Garb}}
\newcommand{\GInput}{\mathsf{GInput}}
\newcommand{\GEval}{\mathsf{Eval}}
\newcommand{\Circuit}{\mathsf{C}}
\newcommand{\hCircuit}{\hat{\mathsf{C}}}
\newcommand{\hFun}{\hat{\mathsf{F}}}
\newcommand{\Fun}{\mathsf{F}}
\newcommand{\GarbledCircuit}{\widetilde{\Circuit}}
\newcommand{\wire}{w}
\newcommand{\inp}{\mathsf{inp}}
\newcommand{\inpsize}{\mathsf{inpsize}}
\newcommand{\out}{\mathsf{out}}
\newcommand{\CircSim}{\mathsf{CircSim}}
\newcommand{\Garbled}[1]{\widetilde{#1}}
\newcommand{\Output}{y}
\newcommand{\Input}{x}
\newcommand{\GarbledInput}{\widetilde x}
\newcommand{\InputKey}{s^{\mathsf{in}}}
\newcommand{\InputSize}{m}
\def\indc{\stackrel{{\tiny{\mathrm{comp}}}}{\approx}}
\newcommand{\RE}{\mathsf{RE}}
\newcommand{\REenc}{\mathsf{RE.enc}}
\newcommand{\REdec}{\mathsf{RE.dec}}

\newcommand{\HandleEval}{\mathtt{HandleEval}}
\newcommand{\ConstructHelpers}{\mathtt{ConstHelp}}
\newcommand{\Reduct}{\mathtt{SecurityRed}}
\newcommand{\Reduc}{\Reduct}

% Algorithms
\newcommand{\scheme}{\mathcal{E}}
\newcommand{\newScheme}{\dot{\scheme}}
\newcommand{\newSchemex}{\ddot{\scheme}}
\newcommand{\newG}{\dot{G}}
\newcommand{\newE}{\dot{E}}
\newcommand{\newD}{\dot{D}}
\newcommand{\newpk}{\dot{pk}}
\newcommand{\newsk}{\dot{sk}}
\newcommand{\newc}{\dot{c}}
\newcommand{\newGx}{\ddot{G}}
\newcommand{\newEx}{\ddot{E}}
\newcommand{\newDx}{\ddot{D}}
\newcommand{\newpkx}{\ddot{pk}}
\newcommand{\newskx}{\ddot{sk}}
\newcommand{\newcx}{\ddot{c}}
\newcommand{\newp}{\dot{p}}
\newcommand{\newpx}{\ddot{p}}
\newcommand{\newq}{\dot{q}}
\newcommand{\newqx}{\ddot{q}}


% Events Notation
\newcommand{\Bad}{\mathrm{Bad}}
\newcommand{\Miss}{\mathrm{Miss}}
\newcommand{\Hit}{\mathrm{Hit}}
\newcommand{\Disjoint}{\mathrm{Disjoint}}

% Query Set Notation
\newcommand{\sets}[1]{\mathsf{#1}}
\newcommand{\Q}[2]{(#2 \xrightarrow[#1]{} \; ?)}
\newcommand{\QA}[3]{(#2 \xrightarrow[#1]{} #3)}
\newcommand{\OrigG}{\sets{OrigG}}
\newcommand{\OrigE}{\sets{OrigE}}
\newcommand{\OrigD}{\sets{OrigD}}
\newcommand{\LearnG}{\sets{LearnG}}
\newcommand{\LocalE}{\sets{LocalE}}
\newcommand{\AllE}{\sets{AllE}}
\newcommand{\LocalD}{\sets{LocalD}}
\newcommand{\EvalD}{\sets{EvalD}}
\newcommand{\SO}{S}
\newcommand{\HintGEnc}{\sets{H}}
\newcommand{\HintGEnci}[1]{\sets{H}^{#1}_{\newE}}
\newcommand{\HintEDec}{\sets{H}}
\newcommand{\HintEDeci}[1]{\sets{H}^{#1}_{\newDx}}
\newcommand{\HintGEncSim}{\HintGEnc^*}
\newcommand{\HintEDecSim}{\HintEDec^*}
\newcommand{\OrigESim}{\sets{\OrigE^*}}
\newcommand{\LocalESim}{\sets{\LocalE^*}}
\newcommand{\LearnGSim}{\LearnG}
\newcommand{\EvalDSim}{\EvalD^*}
\newcommand{\QueryDist}[1]{\mathrm{Query}(#1)}
\newcommand{\AllDist}{DistGen_1}
\newcommand{\Diff}{\sets{Diff}}


\newcommand{\dhat}[1]{\wh{\wh{#1}}}


\newcommand{\tmclass}{\fclass}
\newcommand{\Sim}{\mathsf{Sim}}
\newcommand{\ext}{^{\mathsf{ext}}}

\newcommand{\MSK}{\mathsf{MSK}}
\newcommand{\MPK}{\mathsf{MPK}}
\newcommand{\ID}{f}
\newcommand{\nand}{\barwedge}

\newcommand{\fclass}{\cF}
\newcommand{\secp}{\mathrm{\kappa}}
\newcommand{\secpar}{\secp}

%\newcommand{\Samp}{\mathsf{OnSam}}

\newcommand{\Sam}{\mathsf{Sam}}

%\newcommand{\Att}{\textsc{Attack}}
\newcommand{\Hyb}{\textsc{Hybrid}}
\newcommand{\Idl}{\textsc{Ideal}}
\newcommand{\Lzy}{\textsc{Lazy}}

\newcommand{\HIT}{\mathsf{HIT}}
\newcommand{\MAL}{\mathsf{MAL}}
\newcommand{\INT}{\mathsf{INT}}

\newcommand{\sm}{\setminus}
%\newcommand{\att}{_\mathsf{att}}
\newcommand{\hyb}{_\mathsf{hyb}}
\newcommand{\idl}{_\mathsf{idl}}

\newcommand{\oAtt}{\mathbf{Out}\att}
\newcommand{\oHyb}{\mathbf{Out}\hyb}
\newcommand{\oIdl}{\mathbf{Out}\idl}

\newcommand{\bHyb}{B_\mathsf{hyb}}
\newcommand{\bAtt}{B_\mathsf{att}}

\newcommand{\chal}{\mathbf{chal}}
\newcommand{\gen}{\mathbf{gen}}

\newcommand{\Clsr}{\CLSR}

\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}

\newcommand{\BadE}{\mathsf{BE}} % bad event

% keys mathsf
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\SK}{\mathsf{SK}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\PK}{\mathsf{PK}}
\newcommand{\dk}{\mathsf{dk}}
\newcommand{\DK}{\mathsf{DK}}
\newcommand{\problem}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Rplus}{\R_+}
\newcommand{\Loss}{\mathrm{Risk}}
\newcommand{\loss}{\ell\mathrm{oss}}
% algorithms mahtbf
\newcommand{\e}{\mathrm{e}}
\newcommand{\E}{\mathrm{E}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\id}{\mathbf{id}}
\renewcommand{\D}{\cD}
\newcommand{\g}{\mathbf{g}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\k}{\mathbf{k}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\p}{\mathbf{p}}


\newcommand{\clg}{\ol{\g}}
\newcommand{\clk}{\ol{\k}}
\newcommand{\clid}{\ol{\id}}
\newcommand{\cle}{\ol{\e}}
\newcommand{\cld}{\ol{\d}}



% sets
\newcommand{\atA}{\mathbb{A}}
\newcommand{\atB}{\mathbb{B}}

\newcommand{\prF}{\mathbb{F}}
\newcommand{\prG}{\mathbb{G}}


\newcommand{\PE}{\mathbf{PE}}
\newcommand{\TPE}{\mathbf{TPE}}
\newcommand{\IBE}{\mathbf{IBE}}
\newcommand{\FPE}{\prF\text{-}\PE}
\newcommand{\GPE}{\prG\text{-}\PE}
\newcommand{\tTPE}{\tau\text{-}\TPE}
\newcommand{\ttTPE}{$\tau$-TPE\xspace}

%\newcommand{\att}{\cA}
%\newcommand{\prd}{\cP}
% \usepackage{graphicx}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\newcommand{\remove}[1]{}
\newcommand{\num}[1]{{\bf (#1)}}

\newcommand{\ol}{\overline}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\nin}{\not \in}

\newcommand{\es}{\varnothing} % empty set
\newcommand{\se}{\subseteq}
\newcommand{\nse}{\not \se}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\rv}[1]{\mathbf{#1}} % Random Variable
\newcommand{\rvV}{\rv{V}}




%%%  English %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{et~al.\ }
\newcommand{\aka}{also known as,\ }
\newcommand{\resp}{resp.,\ }
\newcommand{\ie}{i.e.,\ }
\newcommand{\wolog}{w.l.o.g.\ }
\newcommand{\Wolog}{W.l.o.g.\ }
\newcommand{\eg}{e.g.,\ }
\newcommand{\wrt} {with respect to\ }
\newcommand{\cf}{{cf.,\ }}

%%%  math %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\round}[1]{\lfloor #1 \rceil}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\angles}[1]{\langle #1 \rangle}
\newcommand{\parens}[1]{( #1 )}
\newcommand{\bracks}[1]{[ #1 ]}
\newcommand{\bra}[1]{\langle#1\rvert}
\newcommand{\ket}[1]{\lvert#1\rangle}
\newcommand{\set}[1]{\left\{ #1 \right\}}

\newcommand{\adjRound}[1]{\left\lfloor #1 \right\rceil} % Adjusted Round
\newcommand{\adjCeil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\adjFloor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\adjAngles}[1]{\left\langle #1 \right\rangle}
\newcommand{\adjParens}[1]{\left( #1 \right)}
\newcommand{\adjBracks}[1]{\left[ #1 \right]}
\newcommand{\adjBra}[1]{\left\langle#1\right\rvert}
\newcommand{\adjKet}[1]{\left\lvert#1\right\rangle}
\newcommand{\adjSet}[1]{\left\{ #1 \right\}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\quarter}{\tfrac{1}{4}}
\newcommand{\eqdef}{:=}
\newcommand{\zo}{\{0,1\}}
\newcommand{\bits}{\{0,1\}}
\newcommand{\xor}{\oplus}
\newcommand{\tensor}{\otimes}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\,\tiny \$}}{\gets}}}
\newcommand{\from}{\gets}
\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\size{#1}}
%\newcommand{\norm}[1]{\abf{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\To}{\mapsto}
\newcommand{\mcom}{\, ,}
\newcommand{\mper}{\, .}
\newcommand{\sign}{\ensuremath {\pm 1}}
\newcommand{\nbyn}{\ensuremath {n \times n}}
\renewcommand{\L}{\ensuremath L\:}
\newcommand{\LA}{\ensuremath L_A}
\newcommand{\Learn}{\mathsf{Lasso}}
\newcommand{\LASSO}{\mathsf{Lasso}}
\newcommand{\Lasso}{\mathsf{Lasso}}

%%%% Font Abbreviations

\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\F}{{\mathbb F}}

\newcommand{\trainTam}{\vVec}
\newcommand{\Adv}{\mathsf{A}}

\newcommand{\train}{\uVec}
\newcommand{\tamped}[1]{\wh{#1}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

% \usepackage{upgreek}
% \usepackage{bm}

% note the short forms: eps and ups
\newcommand{\bfalpha}{{\bm \alpha}}
\newcommand{\bfbeta}{{\bm \beta}}
\newcommand{\bfgamma}{{\bm \gamma}}
\newcommand{\bfdelta}{{\bm \delta}}
\newcommand{\bfeps}{{\bm \epsilon}}
\newcommand{\bfveps}{{\bm \varepsilon}}
\newcommand{\bfzeta}{{\bm \zeta}}
\newcommand{\bftheta}{{\bm \theta}}
\newcommand{\bfvtheta}{{\bm \vartheta}}
\newcommand{\bfiota}{{\bm \iota}}
\newcommand{\bfkappa}{{\bm \kappa}}
\newcommand{\bflambda}{{\bm \lambda}}
\newcommand{\bfmu}{{\bm \mu}}
\newcommand{\bfnu}{{\bm \nu}}
\newcommand{\bfxi}{{\bm \xi}}
\newcommand{\bfoo}{{\bm \o}}% not to confuse with regular o
\newcommand{\bfpi}{{\bm \pi}}
\newcommand{\bfvarpi}{{\bm \varpi}}
\newcommand{\bfrho}{{\bm \rho}}
\newcommand{\bfvrho}{{\bm \varrho}}
\newcommand{\bfsigma}{{\bm \sigma}}
\newcommand{\bfvsigma}{{\bm \varsigma}}
\newcommand{\bftau}{{\bm \tau}}
\newcommand{\bfups}{{\bm \upsilon}}
\newcommand{\bfphi}{{\bm \phi}}
\newcommand{\bfvphi}{{\bm \varphi}}
\newcommand{\bfchi}{{\bm \chi}}
\newcommand{\bfpsi}{{\bm \psi}}
\newcommand{\bfomega}{{\bm \omega}}


\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}
\newcommand{\eps}{\varepsilon}
%\newcommand{\e}{\epsilon}
\newcommand{\veps}{\varepsilon}
%\newcommand{\vare}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vrho}{\varrho}
\newcommand{\vpi}{\varpi}
\newcommand{\tO}{\widetilde{O}}
\newcommand{\tOmega}{\widetilde{\Omega}}
\newcommand{\tTheta}{\widetilde{\Theta}}
\newcommand{\field}{\ensuremath \Bbbk}
\newcommand{\reals}{\ensuremath \mathbb{R}}
% \DeclareMathOperator{\Rig}{Rig}
% \DeclareMathOperator{\rk}{rank}

% \DeclareMathOperator{\rank}{rank}

%%%%%%%%%%%%%%%% Operators %%%%%%

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\loglog}{\operatorname{loglog}}
\newcommand{\GF}{\operatorname{GF}}
\newcommand{\Exp}{\operatorname*{\mathbb{E}}}
\newcommand{\Ex}{\Exp}
%\newcommand{\view}{\operatorname{view}}
\newcommand{\View}[1]{\mathsf{View}\angles{#1}}
\newcommand{\Var}{\operatorname*{\mathbb{V}}}
\newcommand{\ShH}{\operatorname{H}}
\newcommand{\maxH}{\operatorname{H_0}}
\newcommand{\minH}{\operatorname{H_{\infty}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\Setup}{\operatorname{Setup}}
\newcommand{\KGen}{\operatorname{KGen}}
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\Sign}{\operatorname{Sign}}
\newcommand{\Ver}{\operatorname{Ver}}
\newcommand{\Gen}{\operatorname{Gen}}
\newcommand{\negl}{\operatorname{negl}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\maj}{\operatorname*{maj}}
\newcommand{\argmax}{\operatorname*{argmax}}
\newcommand{\argmin}{\operatorname*{argmin}}
\newcommand{\Image}{\operatorname{Im}}


%%% Computational Problems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\SAT}{\mathrm{SAT}}
\newcommand{\UNSAT}{\mathrm{UNSAT}}
%\newcommand{\ED}{\mathrm{ED}} % Entropy Difference
%\newcommand{\GapSVP}{\mathrm{GapSVP}}
%\newcommand{\GapSIVP}{\mathrm{GapSIVP}}
%\newcommand{\GapCVP}{\mathrm{GapCVP}}
%\newcommand{\COLOR}{\mathrm{3COL}}

%%% Complexity Classes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\class}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\coclass}[1]{\class{co\mbox{-}#1}} %  their complements
\newcommand{\prclass}[1]{\class{Pr#1}}
\newcommand{\PPT}{\class{PPT}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NC}{\class{NC}}
\newcommand{\AC}{\class{AC}}
\newcommand{\NP}{\ensuremath{\class{NP}}}
\newcommand{\coNP}{\ensuremath{\coclass{NP}}}
\newcommand{\RP}{\class{RP}}
\newcommand{\coRP}{\coclass{RP}}
\newcommand{\ZPP}{\class{ZPP}}
\newcommand{\IP}{\class{IP}}
\newcommand{\coIP}{\coclass{IP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\coAM}{\class{coAM}}
\newcommand{\MA}{\class{MA}}
\renewcommand{\P}{\class{P}}
\newcommand\prBPP{\prclass{BPP}}
\newcommand\prRP{\prclass{RP}}
%\newcommand\prP{\prclass{P}}
\newcommand{\Ppoly}{\class{P/poly}}
\newcommand{\DTIME}{\class{DTIME}}
\newcommand{\ETIME}{\class{E}}
\newcommand{\BPTIME}{\class{BPTIME}}
\newcommand{\AMTIME}{\class{AMTIME}}
\newcommand{\coAMTIME}{\class{coAMTIME}}
\newcommand{\NTIME}{\class{NTIME}}
\newcommand{\coNTIME}{\class{coNTIME}}
\newcommand{\AMcoAM}{\class{AM} \cap \class{coAM}}
\newcommand{\NPcoNP}{\class{N} \cap \class{coN}}
\newcommand{\EXP}{\class{EXP}}
\newcommand{\SUBEXP}{\class{SUBEXP}}
\newcommand{\qP}{\class{\wt{P}}}
\newcommand{\PH}{\class{PH}}
\newcommand{\NEXP}{\class{NEXP}}
\newcommand{\PSPACE}{\class{PSPACE}}
%\newcommand{\E}{\class{E}}
\newcommand{\NE}{\class{NE}}
\newcommand{\coNE}{\class{coNE}}
\newcommand{\SharpP}{\class{\#P}}
\newcommand{\prSZK}{\prclass{SZK}}
\newcommand{\BPPSZK}{\BPP^{\SZK}}
\newcommand{\TFAM}{\class{TFAM}}
\newcommand{\RTFAM}{{\R\text{-}\class{TUAM}}}
% relations decidable by a randomized algorithm
\newcommand{\FBPP}{\class{BPP}}
% relations decidable by a RTFAM oracle
\newcommand{\BPPR}{\FBPP^{\RTFAM}}
\newcommand{\TFNP}{\mathbf{TFNP}}
\newcommand{\MIP}{\mathbf{MIP}}
% zero-knowledge complexity classes
\newcommand{\ZK}{\class{ZK}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\SZKP}{\class{SZKP}}
\newcommand{\SZKA}{\class{SZKA}}
\newcommand{\CZKP}{\class{CZKP}}
\newcommand{\CZKA}{\class{CZKA}}
\newcommand{\coSZKP}{\coclass{SZKP}}
\newcommand{\coSZKA}{\coclass{SZKA}}
\newcommand{\coCZKP}{\coclass{CZKP}}
\newcommand{\coCZKA}{\coclass{CZKA}}
\newcommand{\NISZKP}{\class{NI\mbox{-}SZKP}}
\newcommand{\phcc}{\ensuremath \PH^{\mathrm{cc}}}
\newcommand{\pspacecc}{\ensuremath \PSPACE^{\mathrm{cc}}}
\newcommand{\sigcc}[1]{\ensuremath \class{\Sigma}^{\mathrm{cc}}_{#1}}
\newcommand{\aco}{\ensuremath \AC^0}
\newcommand{\ncone}{\ensuremath \NC^1}

%%%%% Theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\ifllncs
\newtheorem{aclaim}{Claim}
%\fi


\newtheorem{theorem}{Theorem}%[section]
% \theoremstyle{plain}
\newtheorem{claim}{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
% \theoremstyle{definition}

\newtheorem{definition}{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{algorithm1}[theorem]{Algorithm}
%\newtheorem{protocol}[theorem]{Protocol} defined below
\newtheorem{assumption}[theorem]{Assumption}

% \theoremstyle{definition}
\newtheorem*{remark}{Remark}
\newtheorem{note}[theorem]{Note}


% Protocol env
\newcommand{\sdotfill}{\textcolor[rgb]{0.8,0.8,0.8}{\dotfill}} %change to \cdotfill later
\newenvironment{protocol}{\begin{proto}}{\vspace{-\topsep}\sdotfill\end{proto}}

\makeatletter
\def\th@protocol{%
    \normalfont % body font
    \setbeamercolor{block title example}{bg=orange,fg=white}
    \setbeamercolor{block body example}{bg=orange!20,fg=black}
    \def\inserttheoremblockenv{exampleblock}
  }
\makeatother
% \theoremstyle{protocol}

\newtheorem{proto}[theorem]{Protocol}
\newtheorem{protoc}[theorem]{Protocol}
\newenvironment{protocolS}{\begin{protoc}}{\vspace{-\topsep}\sdotfill\end{protoc}}

% state/restate
\newcommand{\namedref}[2]{#1~\ref{#2}}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{\namedref{#1}{#2}}
}

\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}

%%% refs macros (hopefully will help in transforming to pdf) %%%%%%


\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
\newcommand{\sectionref}[1]{Sect.~\ref{#1}}
\newcommand{\definitionref}[1]{Definition~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\stepref}[1]{Step~\ref{#1}}
\newcommand{\figureref}[1]{Fig.~\ref{#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\newcommand{\claimref}[1]{Claim~\ref{#1}}
\newcommand{\remarkref}[1]{Remark~\ref{#1}}
\newcommand{\corollaryref}[1]{Corollary~\ref{#1}}
\newcommand{\inequalityref}[1]{Inequality~\ref{#1}}
\newcommand{\constructionref}[1]{Construction~\ref{#1}}
\newcommand{\itemref}[1]{Item~\ref{#1}}
\newcommand{\propertyref}[1]{Property~\ref{#1}}
\newcommand{\protocolref}[1]{Protocol~\ref{#1}}
\newcommand{\algorithmref}[1]{Algorithm~\ref{#1}}
\newcommand{\appendixref}[1]{Appendix~\ref{#1}} 

==> sections/cross_entropy_loss.tex <==
% Here, we calculate the coordinatewise lipschitz constant for the gradient of a single layer neural network with a softmax operator and cross entropy loss. That is, we have a input space $X\in[0,1]^m$ and a $N$ classes. For model $\theta\in \R^{N\times m}$, on an input $x\in X$ the output will be a an $N$-dimensional prediction vector $p$ that is defined as follows:

% $$p_i= \frac{e^{\theta[i]\cdot x}}{\sum_{z\in[N]}{e^{\theta[z]\cdot x}}}$$

% Thus, the single layer neural network can be written as a function $f(x,\theta) = \sigma(\theta^t x)$, where $\sigma(.)$ is the softmax function. We use $\mathrm{CE}$ to denote the cross entropy loss.
% We use $g(x,\theta)$ to denote  $\frac{\partial  \mathrm{CE}(f(x,\theta))}{\partial \theta}$.

% Our goal is to find a constant $c$ such that:
% \[ \sup_{x,\theta_1, \theta_2} \frac{|| g(x,\theta_2) - g(x,\theta_1)||_\infty}{||\theta_2-\theta_1||_1} \leq c\]

% Calculating function $g$ we have

% $$g(x,\theta)[i][j] = 
% \left\{
% 	\begin{array}{ll}
% 		-x_j \frac{e^{\theta[i]\cdot x}}{\sum_{z\in[N]}{e^{\theta[z]\cdot x}}}  & \mbox{if } i \neq y, \\
% 		x_j \frac{1}{\sum_{z\in[N]}{e^{\theta[z]\cdot x}}}  & \mbox{if } i = y.
% 	\end{array}
% \right.$$

% Now define a function $g'=\frac{\partial g}{\partial \theta}$, gradient calculation gives us the following:


% $$g'(x,\theta)[i][j][i'][j'] = 
% \left\{
% 	\begin{array}{ll}
% 		-x_jx_{j'} \frac{\sum_{z\neq i}{e^{\theta[z]\cdot x}}}{(\sum_{z\in[N]}{e^{\theta[z]\cdot x}})^2}  & \mbox{if } i \neq y \mbox{ and } i' = i, \\
% 		x_jx_{j'} \frac{e^{\theta[i]\cdot x}}{(\sum_{z\in[N]}{e^{\theta[z]\cdot x}})^2}  & \mbox{if } i \neq y \mbox{ and } i' \neq i.\\
% 		-x_jx_{j'} \frac{1}{(\sum_{z\in[N]}{e^{\theta[z]\cdot x}})^2}  & \mbox{if } i = y \mbox{ and } i' = i.
		
% 	\end{array}
% \right.$$
% In the following, we outline the set of steps for computing the coordinate-wise Lipschitz constant of the model update with respect to the model parameters for a single layer neural network with softmax cross entropy loss. The model is trained using SGD.
% The input is of the form of $(x, y)$ where $x \in [0, 1]^m$ and $y \in \{0, 1\}^C$ is the one-hot encoded representation of any of the $C$ classes. The model parameters are denoted by $\theta \in \mathbb{R}^{C \times m}$, and the softmax layer by the function $\sigma(\cdot)$. The neural network can thus be represented as $f(x, \theta) = \sigma(\theta x)$.

% We define $g(x, \theta) = \frac{\partial \mathcal{L}(f(x, \theta), y)}{\partial \theta}$ where $\mathcal{L}$ is the cross entropy loss function. Our goal is to find a Lipschitz constant $L$ such that 
% \begin{equation}
% \sup_{x, \theta_1, \theta_2} \frac{|| g(x, \theta_1) - g(x, \theta_2) ||_{\infty}}{|| \theta_1 - \theta_2 ||_1} \leq L
% \label{eqn:lc_0}
% \end{equation}


% We define intermediate variable $z = \theta x$ and the neural network output distribution $p = \sigma(z)$, such that both $p, z \in \mathbb{R}^C$. Note, for a given target class $t$, the cross entropy loss function $\mathcal{L}(p, y) = -\log p_t$ where $p_t = \frac{e^{z_t}}{\sum_{j}e^{z^j}}$. Thus, 
% \begin{equation}
%     g(x, \theta)_{{ij}} = \frac{\partial \mathcal{L}}{\partial \theta_{ij}} = \sum_{c=1}^{C} \frac{\partial \mathcal{L}}{\partial z_c} \frac{\partial z_c}{\partial \theta_{ij}}. \label{eqn:lc_1}
% \end{equation}
% Computing the terms of Eqn.~\eqref{eqn:lc_1}, we have
% \[ \frac{\partial \mathcal{L}}{\partial z_c} = p_t - 1 \;\; \mbox{ for } c=t \mbox {; and } \frac{\partial \mathcal{L}}{\partial z_c} = p_c \mbox{ otherwise }\]
% and $\frac{\partial z_c}{\partial \theta_{{ij}}} = x_j$. Thus, 
% \begin{eqnarray}
% g(x, \theta)_{{ij}} & = & x_j (p_t - 1) \;\; \mbox{ for i = t} \nonumber \\ 
% & = & x_j p_i  \;\; \mbox{ for } i \neq t, i = 1, \ldots, C \label{eqn:lc_2}
% \end{eqnarray}
% We compute the Hessian of $g(x, \theta)_{{ij}}$ as:
% \begin{eqnarray}
% \frac{\partial g(x, \theta)_{{ij}}}{\partial \theta_{{kl}}} & = &  x_j p_t (1-p_t) x_l \;\; \mbox{ for } k = t \nonumber \\
% & = & x_j p_k (1 - p_k) x_l \;\; \mbox{ for } k \neq t, k = 1, \ldots, C \label{eqn:lc_3}
% \end{eqnarray}
% The maximum value of the Hessian in Eqn.~\eqref{eqn:lc_3}, occurs at $x_j = x_l = 1$, and $p_t = p_k = \frac{1}{2}$. Thus, \begin{eqnarray}
% \max_{i, j, k, l}\frac{\partial g(x, \theta)_{{ij}}}{\partial \theta_{{kl}}} & \leq &  \frac{1}{4} \;\; \mbox{ for } k = t \nonumber \\
% & \leq & \frac{1}{4} \;\; \mbox{ for } k \neq t, k = 1, \ldots, C \label{eqn:lc_4}
% \end{eqnarray}
% To obtain the Lipschitz constant, we first define the function
% \[ h(t) = g(x, (1-t)\theta_1 + t \theta_2)_{{ij}} \mbox{ where } t \in [0, 1] \]
% Thus, $h(0) = g(x, \theta_1)_{{ij}}$ and $h(1) = g(x, \theta_2)_{{ij}}$. Since, the function $h(t)$ is differentiable everywhere in $(0, 1)$, using Mean Value Theorem~\cite{nla.cat-vn298857}, we know that there exists a point $t^{*}$ such that:
% \begin{equation}
%  |h(1) - h(0)| \leq h'(t^{*}) 
% \mbox{ where } h'(t) = |\theta_2 - \theta_1| g'(x, (1-t) \theta_1 + t \theta_2)_{{ij}}. \label{eqn:lc_5}
% \end{equation}
% Rewriting, Eqn.~\eqref{eqn:lc_0}, we get
% \begin{eqnarray}
% & & \sup_{x, \theta_1, \theta_2} |g(x, \theta_1) - g(x, \theta_2) | \nonumber \\
% & = & \sup_{x, \theta_1, \theta_2} \max_{i, j} |g(x, \theta_1)_{{ij}} - g(x, \theta_2)_{{ij}} | \nonumber 
% \end{eqnarray}
% Without loss of generality, let $i^{*}, j^{*}$ correspond to the indices where the maximum of the above equation occurs. Combining Eqns~\eqref{eqn:lc_4} and \eqref{eqn:lc_5}, we get:
% \begin{equation}
%     \sup_{x, \theta_1, \theta_2} | g(x, \theta_1)_{i^{*} j^{*}} - g(x, \theta_2)_{i^{*} j^{*}} | \leq \frac{1}{4} |\theta_1 - \theta_2|
% \end{equation}
% which completes the proof.
\input{sections/proof}
